High performance Wannier interpolation of Berry curvature and related quantities: WannierBerri code

Wannier interpolation is a powerful tool for performing Brillouin zone integrals over dense grids of $\mathbf{k}$ points, which are essential to evaluate such quantities as the intrinsic anomalous Hall conductivity or Boltzmann transport coefficients. However, new physical problems and new materials create new numerical challenges, and computations with the existing codes become very expensive, which often prevents reaching the desired accuracy. In this article, I present a series of methods that boost the speed of Wannier interpolation by several orders of magnitude. They include a combination of fast and slow Fourier transforms, explicit use of symmetries and recursive adaptive grid refinement among others. The proposed methodology has been implemented in the new python code WannierBerri, which also aims to serve as a convenient platform for the future development of interpolation schemes for novel phenomena.

==> install.tex <==
To run the \wBerri code only python3 is required, independent of the operating system. 
The easy way of installation of the latest stable version maybe achieved via \lstinline{pip}\cite{pypi-wberri}:
\begin{lstlisting}
pip3 install wannierberri
\end{lstlisting}
The dependencies are quite basic and will be installed automatically. Those include \lstinline{numpy}\cite{numpy}, \lstinline{scipy >= 1.0}\cite{scipy}, pyFFTW\cite{pyFFTW} (python wrapper of FFTW\cite{FFTW05}), \lstinline{lazy_property}, and a few 'cosmetic' modules \lstinline{colorama}, \lstinline{termcolor} and \lstinline{pyfiglet} which are needed for a nice colorful output in the terminal. 

One note should be mentioned about the parallel run. numpy already includes parallelization over threads. However, if \wBerri is running with the number of processes equal to the number of physical cores, obviously extra threading may only slow down the calculation. Generally I recommend to switch off the threading in numpy by setting the corresponding environent variable. It can be done inside the python script by 
\begin{lstlisting}
import os
os.environ['OPENBLAS_NUM_THREADS'] = '1'
\end{lstlisting}
or
\begin{lstlisting}
os.environ['MKL_NUM_THREADS'] = '1'  
\end{lstlisting}
Depending whether numpy is linked with openblas or MKL libraries. Note, this should be done in the beginning of the script, before importing numpy for the first time. 


\section{Contributing to the code}
\wanBerri is a free open-source project, nder the GNU public Licence v2, and everyone is welcome to modify the code to better match  one's own needs. Contributions that might be useful for general public are encouraged to be submitted via pull request on gitHub \cite{github-wberri}.





